Beyond Primitive Bloat: High-Fidelity Gaussian Splatting via Coordinate-Convolution Neural Network

Gaussian Splatting (GS) has revolutionized Novel View Synthesis (NVS) with fast training and real-time rendering, yet pushing its fidelity to arbitrary high levels remains an open challenge. We theoretically explain this barrier by proving that discrete Gaussian representations require an exponentially increasing number of primitives to raise training PSNR, which inevitably triggers optimization issues and validation overfitting. To bypass this scaling limit without primitive bloat, we formulate detail recovery as a continuous neural field over coarse renderings and prove that monotonically reducing approximation risk to zero requires jointly leveraging low-fidelity signals, local neighborhood, and coordinate queries. Guided by this result, we augment splatted renderings with an existing Coordinate-Convolution Neural Network (CCNN) that jointly convolves rendered low-fidelity signals with 2D pixel coordinate queries to synthesize residuals. Integrating CCNN into five diverse Gaussian Splatting baselines establishes new state-of-the-art fidelity across NVS benchmarks while preserving real-time rendering speeds with minimal training and storage overhead. Beyond NVS, they also consistently boost performance of 1D/2D regression and 2D super-resolution tasks.

==> preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}
